CORe: Capitalizing On Rewards in Bandit Exploration

We propose a bandit algorithm that explores purely by randomizing its past observations. In particular, the sufficient optimism in the mean reward estimates is achieved by exploiting the variance in the past observed rewards. We name the algorithm Capitalizing On Rewards (CORe). The algorithm is general and can be easily applied to different bandit settings. The main benefit of CORe is that its exploration is fully data-dependent. It does not rely on any external noise and adapts to different problems without parameter tuning. We derive a $\tilde O(d\sqrt{n\log K})$ gap-free bound on the $n$-round regret of CORe in a stochastic linear bandit, where $d$ is the number of features and $K$ is the number of arms. Extensive empirical evaluation on multiple synthetic and real-world problems demonstrates the effectiveness of CORe.

==> core.tex <==
\section{Capitalizing on Rewards in Bandit Exploration}

We present the new algorithm Capitalizing On Rewards (\core) in \cref{alg:core}. In each round $t$, \core constructs a \emph{reward pool} $\mathcal{R}_t$ from all the past $t-1$ observed rewards. Let $T_{i,t} = \sum_{\ell = 1}^t \mathbbm{1}\{I_{\ell}=i\}$ denote the number of pulls of arm $i$ in the first $t$ rounds. To achieve optimism and overestimate the mean reward of arm $i$ in round $t$, each of its past $s = T_{i, t - 1}$ rewards is paired with a reward sampled from $\mathcal{R}_t$ scaled by $\alpha > 0$. Then the estimate of the mean reward of arm $i$, $\hat\mu_{i,t}$, is the average of the arm's own $s$ rewards and $s$ sampled and scaled rewards from $\mathcal{R}_t$. The arm with the highest reward estimate is pulled. This is similar to perturbed history exploration \citep{kveton2019perturbedhistory} and TS \citep{thompson1933on}, which add noise to the mean reward estimate. However, \core does not depend on any external pseudo rewards or posterior variance, and instead only relies on randomness in the agent's history. % In particular, the exploration in \core is caused by perturbing the history of each arm by sampled rewards from $\mathcal R_t$, which is constructed from the agent's past observations, and thus is data-dependent.

Specifically, in lines 3-5 of \cref{alg:core}, we initialize \core by pulling all arms sequentially for the first $\max\{K,\frac{2\log n}{z-1-\log z}\}$ round, where $z\in{(0,1)}$ is a tunable parameter that determines the initial variance in the reward pool. After initialization, in each round $t$, \core processes the past $t-1$ rewards and create the reward pool $\mathcal{R}_t$ in lines 7-10. The processed rewards in $\mathcal{R}_t$ have zero mean and each reward $y$ has its symmetric reward $-y$ around zero in the pool. This additional processing is only for the ease of theoretical analysis in \cref{sec:analysis}. It does not change the variance of samples from the reward pool and \core performs in practice similarly without it. Let $V_{i,s}$ be the cumulative reward of arm $i$ after $s$ pulls. For this arm, \core samples $s$ i.i.d.\ rewards from $\mathcal{R}_t$ (line 13) and scales each of the sampled rewards by $\alpha$. The sum of $s$ sampled and scaled rewards is $U_{i,s}$ (line 14). By estimating the mean reward as in line 15, \core essentially shifts each of the arm's past rewards by a sampled and scaled reward from $\mathcal{R}_t$ and then calculates the average of the shifted rewards. Finally, in lines 18-23, the cumulative reward of the pulled arm and the number of pulls are updated with the newly observed reward $Y_{I_t,t}$.

% \todob{The above description is hard to follow for two reasons:

% 1) We have two reward pools, "reward pool" and "preprocessed reward pool". Clearly name and define these two concepts, and make clear how they relate to each other.
% 2) Separate how we explore and how we guarantee that the reward pool has good properties. A better flow may be the following:
% a) We explore by adding random rewards from "preprocessed reward pool", which is constructured from past observations. This is like a data-dependent follow the perturbed leader / PHE / TS.
% b) "preprocessed reward pool" is just a simple transformation of the "reward pool". Explain why we need it.
% c) We rely on the fact that "reward pool" has sufficient variance, which comes from different pulled arms and reward noise. To guarantee that the reward pool is good, we have a short initialization period that does not depend on the amount of noise. This naturally leads to the next paragraph.}

% We denote the set of all observed rewards so far as the \emph{reward pool} $\mathcal{R}_t = \{Y_{I_\ell, \ell}\}_{\ell = 1}^{t - 1}$. The number of pulls of arm $i$ in the first $t$ rounds is $T_{i,t}=\sum_{\ell}^t\mathbbm{1}\{I_{\ell}=i\}$. We use parameter $z$ to decide the initial variance of the reward pool, \todob{Too many details too early.} and the number of pulls needed for initialization (line 5-6). In round $t$, we first center and mirror the rewards in $\mathcal R_t$ (line 8-10), so that the rewards in the reward pool has zero mean and are symmetric. \todob{This is only needed for the analysis. Present the algorithm in a simpler form.} This step does not influence the mechanism of the algorithm, but is only for the convenience analysis in \cref{sec:analysis}. Then we sample $s$ rewards from the processed reward pool and scale each reward by $\alpha$. \todob{It is not clear what "processed reward pool" is. Either define it or do not use this terminology.} The estimated mean reward is obtained from the sum of the rewards of arm $i$ after $s$ pulls, $V_{i,s}$, and the sum of the sampled and scaled rewards from the reward pool, $U_{i,s}$, i.e., $\hat\mu_{i,s}=(V_{i,s}+U_{i,s})/s$ as shown in line 12-15. The arm with the highest estimated mean will be pulled in this round. Note that scaling each reward sampled from the reward pool by $\alpha$ is equivalent to sample $\alpha^2$ rewards without scaling, and again, this is only for the convenience analysis.  

% \todob{The paragraph below is too complex to parse. Focus on the main idea. We want the reward pool to have a particular property. We initialize it to be close to that property, because we cannot get that property with a high probability just by initialization. To get the property, additionally scale the rewards later. Of course, this is just an outline that needs to be more technical.} 

% The initial variance ratio $z$ means the empirical variance we aim to achieve in the reward pool with respect to the variance of true reward distribution. For example, if the variance of the reward distribution is $\sigma^2$, then we want the empirical variance of the reward pool to be at least $z\sigma^2$. Once $z$ is fixed, the scale ratio $\alpha$ dictates the multiplicative factor of each sampled reward from the reward pool and controls the trade-off between exploration and exploitation. In particular, a larger $\alpha$ will amplify the variance introduced by the sampled rewards and lead to more exploration. More importantly, the variance of sampling from the reward pool depends on the variance of the true reward distribution, i.e., $z\sigma^2$, which automatically is adjusted in different problems. In the next section, we first provide the insight to prove informally that as long as $z\alpha>1$, \core is able to achieve sub-linear regret, agnostic to the problem. 

The exploration in \core arises from the variance of sampled rewards from $\mathcal R_t$. Specifically, if the variance of all reward distributions is $\sigma^2$, we want a comparable variance in $\mathcal R_t$, so that the sampled rewards can offset the underestimated mean rewards of arms due to their unfavorable reward histories. To achieve this, \core initially pulls all arms sequentially $\max\{K,\frac{2\log n}{z-1-\log z}\}$ times, for $z\in(0,1)$, to accumulate observations. We prove in \cref{sec:analysis} that after this initialization, the empirical variance in the reward pool is at least $z\sigma^2/2$ with a high probability. However, $z\sigma^2/2$ may not be sufficient for effective exploration. Once $z$ is fixed, the scale ratio $\alpha$ dictates the multiplicative factor of the variance of each sampled reward, and thus controls the trade-off between exploration and exploitation. Larger $\alpha$ leads to more exploration. More importantly, the variance in $\mathcal R_t$ is at least $z / 2$ of that of the reward distributions. So it is automatically adapted to the problem.

Next we provide an insight on how \core achieves sublinear regret when $\alpha^2z>2$, without knowing the value of $\sigma^2$.

\begin{algorithm}[t]
\caption{Capitalizing on Rewards in a $K$-armed bandit}
\hspace*{\algorithmicindent}\;\textbf{Input}: Initial variance ratio $z\in(0,1)$, sample \\ \hspace*{\algorithmicindent}\; scale ratio $\alpha\in\mathbb R^+$, number of rounds $n$

\begin{algorithmic}[1]
\label{alg:core}
% \STATE \textbf{Initialize}: Reward pool $\mathcal R_1\leftarrow ()$
\FOR{$i=1,2,...,K$}
    \STATE $T_{i,0}\leftarrow 0$, $V_{i,0}\leftarrow 0$
\ENDFOR
\FOR{$t=1,2,...,n$}
    \IF{$t\leq \max\Big\{K, \frac{2\log n}{(z-1-\log z)}\Big\}$}
        \STATE $I_t\leftarrow t \Mod K$
% \STATE Pull arm $I_t$ and get reward $Y_{I_t, t}$
    \ELSE
        % \STATE $\mu(\mathcal{R}_t)=\frac{1}{|\mathcal{R}_t|}\sum_{y\in\mathcal{R}_t}y,\; \mathcal{\tilde R}_t \leftarrow()$ 
        % \FOR{$y\,\text{in}\,\mathcal{R}_t$}
        % \STATE $y\leftarrow y-\mu(\mathcal{R}_t)$, $\mathcal{\tilde R}_t\oplus(y,-y)$
        \STATE $\mathcal{R}_t \gets ()$
        \STATE $\mu(\mathcal{R}_t) = \frac{1}{t - 1} \sum_{\ell = 1}^{t - 1} Y_{I_\ell, \ell}$
        \FOR{$\ell = 1, \dots, t - 1$}
            \STATE $\mathcal{R}_t \gets \mathcal{R}_t \oplus (Y_{I_\ell, \ell} - \mu(\mathcal{R}_t), \, \mu(\mathcal{R}_t) - Y_{I_\ell, \ell})$
        \ENDFOR
% \todob{This is a complicated and imprecive way of writing $\mathcal{\tilde R}_t \gets \mathcal{\tilde R}_t \oplus (y - \mu(\mathcal{R}_t), \mu(\mathcal{R}_t) - y)$.}
% \STATE $\mathcal{\tilde R} \leftarrow$ subtract $\mu$ from each reward in $\mathcal{R}$
% \STATE $\mathcal{\tilde R} \leftarrow$  each reward in $\mathcal{\tilde R}$
        \FOR{$i=1,2,...,K$}
            \STATE $s\leftarrow T_{i,t-1}$
            \STATE $\mathcal{B}_{i,s} \leftarrow$ Sample $s$ i.i.d.\ rewards from $\mathcal{R}_t$
            \STATE $U_{i,s} \leftarrow \sum_{y\in \mathcal{B}_{i,s}}\alpha y$
            \STATE $\hat\mu_{i,t} = \frac{V_{i,s}+U_{i,s}}{s}$
        \ENDFOR
        \STATE $I_t\leftarrow \arg\max_{i\in [K]}\hat\mu_{i,t}$
    \ENDIF
    \STATE Pull arm $I_t$ and get reward $Y_{I_t,t}$
    \FOR{$i=1,2,...,K$} 
        \IF{$i = I_t$}
            \STATE $T_{i,t} \leftarrow T_{i,t-1}+1$ 
            \STATE $V_{i,T_{i,t}} \leftarrow V_{i,s} + Y_{I_t,t}$ 
            % \STATE $\mathcal{R}_{t+1} \leftarrow \mathcal{R}_t \oplus (Y_{I_t,t})$ \todob{Is $\mathcal{R}_t$ is a set or a vector? I am asking because you defined $\mathcal{R}_t$ as the set at the beginning of this section.}
        \ELSE 
            \STATE $T_{i,t} \leftarrow T_{i,t-1}$ 
        \ENDIF
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}


\subsection{Informal Justification of \core}
\label{sec:informal}
To illustrate how \core ensures effective exploration, we make an analogy between \core and \ts. For example, in a Gaussian bandit, adding additive noise to the mean reward estimate is equivalent to posterior sampling. 

In particular, fix arm $i$ and the number of its pulls $s$. Let $\mu_i\sim\mathcal N(\mu_0,\sigma^2)$ be the mean reward of arm $i$, where $\mathcal N(\mu_0,\sigma^2)$ is the Gaussian prior in \ts and $\sigma^2$ is the variance of the arm's reward distribution. Let $(Y_{i,\ell})_{\ell=1}^s \sim \mathcal N(\mu_i,\sigma^2)$ be $s$ i.i.d.\ noisy observations of $\mu_i$. Then the posterior distribution of $\mu_i$ conditioned on $(Y_{i,\ell})_{\ell=1}^s$ is 
\begin{equation}
\label{eq:posterior}
    \mathcal N\Bigg(\frac{\mu_0+\sum_{\ell=1}^sY_{i,\ell}}{s+1}, \frac{\sigma^2}{s+1}\Bigg).
\end{equation}
It is well known that sampling from this distribution in \ts leads to near-optimal regret \citep{agrawal2013furtherTS}. From another perspective, sampling a mean reward of arm $i$ as above is equivalent to adding i.i.d.\ Gaussian noise to $\mu_0$ and each reward in $(Y_{i,\ell})_{\ell=1}^s$, and then taking the average \citep{kveton2019perturbedhistory}. Specifically,
\begin{equation*}
    \frac{\mu_0+Z_0 + \sum_{\ell=1}^{s}(Y_{i,\ell}+Z_\ell)}{s+1}
\end{equation*}
is a sample from distribution \eqref{eq:posterior} for $(Z_\ell)_{\ell=0}^s\sim\mathcal N(0,\sigma^2)$.

However, in practice, $\sigma^2$ depends on the specific problem instance and is unknown. Thus the variance of $(Z_\ell)_{\ell=0}^s$ needs to be carefully tuned to match $\sigma^2$. The key insight in this work is that the exact value of $\sigma^2$ does not have to be known. Instead of sampling the noise from a given distribution, \core samples $(Z_{l})_{\ell=0}^s$ from the reward pool $\mathcal R_t$ and adds it to each observed reward. As we show in \cref{sec:analysis}, after the initialization in \core, the empirical variance in the reward pool is at least $z\sigma^2/2$ with a high probability, proportional to $\sigma^2$ by a factor of $z/2$. Thus, after scaling the rewards from $\mathcal R_t$ by $\alpha$, the variance of each i.i.d.\ sampled reward is greater than $\alpha^2z\sigma^2/2$. This is at least $\sigma^2$ for $\alpha^2 z > 2$, and can be achieved without knowing $\sigma^2$. 

%%% below are commented
\begin{comment}
Fix arm $i$ and the number of its pulls $s$. Let $V_{i,s}$ be the cumulative reward of arm $i$ after $s$ pulls, and $U_{i,s}$ be the sum of $s$ sampled rewards from the reward pool $\mathcal{R}_t$ %, where the rewards have zero mean and for each reward $y$, there is a $-y$ so that the rewards are symmetric according to zero. % \todob{Formally define $U_{i, s}$. The current description is too blah blah blah.}
% \todob{It is not clear what "symmetric according to zero" is.} 
Then the estimated mean reward of arm $i$ is 
\begin{equation}
\label{eq:mean}
    \hat\mu_{i} = \frac{V_{i,s}+U_{i,s}}{s}.
\end{equation}
First, it is easy to argue the convergence of the estimated mean to the true mean when $s$ increases. Let $\bar V_{i,s} = \E{V_{i,s}}$, $\bar U_{i,s}= \E{U_{i,s}}$, and the variance of the true reward distribution be $\sigma^2$, we have
\begin{equation}
    \mathbb E[\hat\mu_{i}] = \frac{\bar V_{i,s} + \bar U_{i,s}}{s} =  \frac{s\mu_i+0}{s} = \mu_i.
\end{equation}
Besides, the observed rewards in the reward pool is always bounded. Thus $\var{U_{i,s}/s}$ is also bounded and $\var{V_{i,s}/s} = \sigma^2/s$, which ensures the convergence of the mean estimate. 

% \todob{Define macros for variance and std. How about $\var{X}$ and $\std{X}$? The macros are above.}

Second, we show that $\hat\mu_i$ is a sufficiently optimistic estimate given arm $i$'s unfavorable reward history. Specifically, let $E=\{\bar V_{i,s}/s-V_{i,s}/s=\varepsilon\}$ be the event that the estimated mean reward of arm $i$ after $s$ pulls is below the expected mean reward by $\varepsilon>0$. Then  $\hat\mu_i$ is an optimistic estimate if
\begin{equation}
\label{eq:optimism}
    \condprob{\frac{V_{i,s}+U_{i,s}}{s} \geq \frac{\bar V_{i,s}+ \bar U_{i,s}}{s}}{E} > \prob{E}
\end{equation}
for any $\varepsilon>0$ such that $\prob{E}>0$. This means that when the empirical mean reward of arm $i$ deviates from the expected mean by $\varepsilon$, the conditional probability of the estimated mean $\hat\mu_i$ being as high as the true mean $\mu_i$ is higher than the probability of this deviation. Under this condition, \core has effective exploration and can offset potential unfavorable deviations.

To prove this informally, first note that: 
\begin{equation}
    \prob{\frac{\bar V_{i,s}-V_{i,s}}{s} \geq \varepsilon} \geq \prob{E}
\end{equation}
holds trivially for any $\varepsilon$. Therefore, if both $\hat\mu_i$ and $V_{i,s}/s$ are normally distributed and $\var{\hat\mu_i|V_{i,s}}>\var{V_{i,s}/s}$ for any $V_{i,s}$, the inequality \ref{eq:optimism} will be satisfied. Recall that after initialization, the empirical variance in the reward pool is at least $z\sigma^2/2$ with high probability. Thus 
\begin{equation}
    \var{\hat\mu_i|V_{i,s}}=\var{\frac{U_{i,s}}{s}} \geq \frac{\alpha^2z\sigma^2}{2s}. 
\end{equation}
As long as $\alpha^2z>2$, $\hat\mu_i$ is an optimistic estimate. We formally prove this intuition in \cref{sec:analysis} to address the assumptions. We will show in the experiments that this is a very loose argument, and \core is able to perform well with much softer requirements than $\alpha^2z>2$.
\end{comment}

